CAT: Change-focused Android GUI Testing

Android Apps are frequently updated, every couple of weeks, to keep up with changing user, hardware and business demands. Correctness of App updates is checked through extensive testing. Recent research has proposed tools for automated GUI event generation in Android Apps. These techniques, however, are not efficient at checking App updates as the generated GUI events do not prioritise updates, and instead explore other App behaviours. We address this need in this paper with CAT (Change-focused Android GUI Testing). For App updates, at the source code or GUI level, CAT performs change impact analysis to identify GUI elements affected by the update. CAT then generates length-3 GUI event sequences to interact with these GUI elements. Our empirical evaluations using 21 publicly available open source Android Apps demonstrated that CAT is able to automatically identify GUI elements affected by App updates, generate and execute length-3 GUI event sequences focusing on change-affected GUI elements. Comparison with two popular GUI event generation tools, DroidBot and DroidMate, revealed that CAT was more effective at interacting with the change-affected GUI elements. Finally, CAT was able to detect previously unknown change-related bugs in two Apps.

==> abstract_formatted.tex <==
Android Apps are frequently updated, every couple of weeks, to keep up with changing user, hardware and business demands. Correctness of App updates is checked through extensive testing. Recent research has proposed tools for automated GUI event generation in Android Apps. These techniques, however, are not efficient at checking App updates as the generated GUI events do not prioritise updates, and instead explore other App behaviours.

We address this need in this paper with CAT (Change-focused Android GUI Testing). For App updates, at the source code or GUI level, CAT performs change impact analysis to identify GUI elements affected by the update. CAT then generates length-3 GUI event sequences to interact with these GUI elements. Our empirical evaluations using 21 publicly available open source Android Apps demonstrated that CAT is able to automatically identify GUI elements affected by App updates, generate and execute length-3 GUI event sequences focusing on change-affected GUI elements. Comparison with two popular GUI event generation tools, DroidBot and DroidMate, revealed that CAT was more effective at interacting with the change-affected GUI elements. Finally, CAT was able to detect previously unknown change-related bugs in two Apps.

==> backupfigure.tex <==

\pgfplotstableread{
    sharp droidmate  droidbot cat
    1	1000	561	18
    2	1000	442	64
    3	54	57	80
    4	124	108	36
    5	1000	132	58
    6	70	5	5
    7	386	131	7
    }\tablecolumnOnePartOne
    
    \pgfplotstableread{
    sharp droidmate  droidbot cat
    8	1000	1000	1000
    9	79	1000	38
    10	858	667	32
    11	207	848	124
    12	1000	44	5
    13	1000	231	37
    14	308	378	46
    }\tablecolumnOnePartTwo
    
    \pgfplotstableread{
    sharp droidmate  droidbot cat
    15	1000	215	22
    16	1000	77	12
    17	82	82	39
    18	1000	238	45
    19	1000	46	19
    20	375	889	896
    21	298	281	73
    }\tablecolumnOnePartThree
    
    \pgfplotstableread{
        sharp droidmate droidbot cat
        1	0	10.0	35.6
        2	0	10.0	46.2
        3	12.5	6.1	19.0
        4	12.9	8.1	39.5
        5	0	22.2	69.6
        6	12.0	10.0	82.6
        7	8.3	10.0	54.5
        8	0.0	0	0
        9	15.4	0.0	35.3
        10	1.2	1.5	33.7
        11	18.2	50.0	100.0
        12	0.0	4.3	36.2
        13	0.0	1.0	34.9
        14	5.9	3.9	58.2
        15	0.0	3.6	36.9
        16	0.0	7.0	23.4
        17	7.8	27.4	57.1
        18	0.0	2.2	32.8
        19	0	9.5	78.0
        20	30.8	50.0	100.0
        21	8.0	3.7	62.8
    }\tablecolumnTwo
    
    \begin{figure*}[!htbp]
        \centering
        \setlength{\tabcolsep}{1pt}
        \setlength{\extrarowheight}{20pt}
        \scriptsize
        \begin{tabular}[t]{ccc}
                \begin{tikzpicture}
                    \begin{axis}[
                        axis x line*=top,
                        axis y line*=left,
                        width=0.32\textwidth,
                        height=0.65\textwidth,
                        xbar,
                        ymin=1,
                        ymax=7,
                        ylabel={App \#},
                        y label style={at={(0.1, 0.5)}},
                        symbolic y coords={1, 2, 3, 4, 5, 6, 7},
                        ytick=data,
                        nodes near coords,
                        every node near coord/.append style={font=\scriptsize},
                        enlarge x limits={upper, value=0.1},
                        enlarge y limits=0.1,
                    ]
                    \addplot
                        table[y=sharp,x=droidmate] {\tablecolumnOnePartOne};
                    \addplot
                        table[y=sharp,x=droidbot] {\tablecolumnOnePartOne};
                    \addplot
                        table[y=sharp,x=cat] {\tablecolumnOnePartOne};
                \legend{}
                \end{axis}
                \end{tikzpicture}
    
    
            &
    
                \begin{tikzpicture}
                    \begin{axis}[
                        width=0.32\textwidth,
                        height=0.65\textwidth,
                        axis x line*=top,
                        axis y line*=left,
                        xbar,
                        ymin=8,
                        ymax=14,
                        ylabel={},
                        symbolic y coords={8, 9, 10, 11, 12, 13, 14},
                        ytick=data,
                        nodes near coords,
                        every node near coord/.append style={font=\scriptsize},
                        enlarge x limits={upper, value=0.1},
                        enlarge y limits=0.1,
                        ]
                    \addplot
                        table[y=sharp,x=droidmate] {\tablecolumnOnePartTwo};
                    \addplot
                        table[y=sharp,x=droidbot] {\tablecolumnOnePartTwo};
                    \addplot
                        table[y=sharp,x=cat] {\tablecolumnOnePartTwo};
                \legend{}
                \end{axis}
                \end{tikzpicture}
    
            &
    
                \begin{tikzpicture}
                    \begin{axis}[
                        width=0.32\textwidth,
                        height=0.65\textwidth,
                        axis x line*=top,
                        axis y line*=left,
                        xbar,
                        ymin=15,
                        ymax=21,
                        ylabel={},
                        symbolic y coords={15, 16, 17, 18, 19, 20, 21},
                        legend style={at={(1,0.68)},anchor=north east},
                        y dir=reverse,
                        ytick=data,
                        nodes near coords,
                        every node near coord/.append style={font=\scriptsize},
                        enlarge x limits={upper, value=0.22},
                        enlarge y limits=0.1,
                        ]
                    \addplot
                        table[y=sharp,x=droidmate] {\tablecolumnOnePartThree};
                    \addplot
                        table[y=sharp,x=droidbot] {\tablecolumnOnePartThree};
                    \addplot
                        table[y=sharp,x=cat] {\tablecolumnOnePartThree};
                    \legend{DroidMate,DroidBot,CAT},
                \end{axis}
                \end{tikzpicture}
    
        \end{tabular}
        %\vspace{-10pt}
        \caption{Number of events used by each tool before the first interaction with target GUI elements.}
        %\vspace{-10pt}
        \label{fig:tableColumnOne}
    \end{figure*}
    
    \begin{figure*}
        \centering
        \scriptsize
        \begin{tikzpicture}
            \begin{axis}[
                width=\textwidth,
                height=0.35\textwidth,
                ybar=0pt,
                xtick distance=1,
                clip=false,
                enlargelimits=false,
                axis x line*=bottom,
                axis y line*=left,
                enlargelimits=0.15,
                legend style={at={(0.5,1.1)},
                    anchor=north,legend columns=-1},
                xlabel={App \#},
                ylabel={Percentage \%},
                y label style={at={(0.041, 0.5)}},
                ymin=0,
                ymax=100,
                every node near coord/.append style={font=\scriptsize},
                xtick=data,
                nodes near coords,
                nodes near coords align={vertical},
                enlarge x limits=0.1,
                enlarge y limits=0.1,
                ]
                \addplot
                table[x=sharp,y=droidmate] {\tablecolumnTwo};
            \addplot
                table[x=sharp,y=droidbot] {\tablecolumnTwo};
            \addplot
                table[x=sharp,y=cat] {\tablecolumnTwo};
            \legend{DroidMate,DroidBot,CAT}
            \end{axis}
        \end{tikzpicture}
        \caption{Percentage of target state events interacting with the target GUI element}
        \label{fig:tableColumnTwo}
    
    \end{figure*}
